Financial Numeric Extreme Labelling: A Dataset and Benchmarking for XBRL Tagging

The U.S. Securities and Exchange Commission (SEC) mandates all public companies to file periodic financial statements that should contain numerals annotated with a particular label from a taxonomy. In this paper, we formulate the task of automating the assignment of a label to a particular numeral span in a sentence from an extremely large label set. Towards this task, we release a dataset, Financial Numeric Extreme Labelling (FNXL), annotated with 2,794 labels. We benchmark the performance of the FNXL dataset by formulating the task as (a) a sequence labelling problem and (b) a pipeline with span extraction followed by Extreme Classification. Although the two approaches perform comparably, the pipeline solution provides a slight edge for the least frequent labels.

==> Sections/Analysis.tex <==
 

==> Sections/Discussion.tex <==
% \section{Discussion}
% \subsection{Why is this a challenging problem?}
% As of 2021, SEC document contained around 20323 labels in total. While many of these labels refer to tabular items or text blocks, there are still many relevant 

==> Sections/ProblemFormulation.tex <==
\section{Problem Formulation}

We define the problem as, given a sentence, identifying the relevant numerals and assigning them a particular US-GAAP label. For example, for a sentence "At December 31, 2020, the Company reported \$929.3 million of trade receivables, net of allowances of \$21.0 million.", the task is to identify the numerals and label them with their appropriate label. In this sentence, the numeral $\textbf{929.3}$ is tagged as \textit{"Receivables Net Current"} and $\textbf{21.0}$ is tagged as \textit{"Allowance For Doubtful Accounts Receivable"}.



% This problem setting is comparable to the Named Entity Recognition(NER) problem setting, however, NER models typically classify a span into a limited number of labels. We showcase the poor performance of NER models through experiments using the \finer setting. To overcome this problem, we introduce a pipeline solution which first identifies the relevant numerals using a sequence-to-sequence tagger and then attempts to assign a label to the relevant numeral.


